Improper Reinforcement Learning with Gradient-based Policy Optimization

We consider an improper reinforcement learning setting where a learner is given $M$ base controllers for an unknown Markov decision process, and wishes to combine them optimally to produce a potentially new controller that can outperform each of the base ones. This can be useful in tuning across controllers, learnt possibly in mismatched or simulated environments, to obtain a good controller for a given target environment with relatively few trials. \par We propose a gradient-based approach that operates over a class of improper mixtures of the controllers. We derive convergence rate guarantees for the approach assuming access to a gradient oracle. The value function of the mixture and its gradient may not be available in closed-form; however, we show that we can employ rollouts and simultaneous perturbation stochastic approximation (SPSA) for explicit gradient descent optimization. Numerical results on (i) the standard control theoretic benchmark of stabilizing an inverted pendulum and (ii) a constrained queueing task show that our improper policy optimization algorithm can stabilize the system even when the base policies at its disposal are unstable\footnote{Under review. Please do not distribute.}.

==> fig_queueing_motivation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
% SYNTAX: \resizebox{width}{height}
\resizebox{9.50cm}{3.75cm}{

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,273); %set diagram left start at 0, and has height of 273

%Straight Lines [id:da09715700995858345] 
\draw [line width=1.5]    (81.8,155.36) -- (260.8,155.36) ;
%Straight Lines [id:da8887479227991981] 
\draw [line width=1.5]    (80.8,215.36) -- (260.8,216.36) ;
%Straight Lines [id:da6217209993953612] 
\draw    (61.8,185.36) -- (89.8,185.36) ;
\draw [shift={(91.8,185.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da875509031522369] 
\draw [line width=1.5]    (260.8,155.36) -- (260.8,216.36) ;
%Straight Lines [id:da37671038244024846] 
\draw    (180,45) -- (257.8,45) ;
\draw [shift={(260.8,45)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(177,45)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0678614898035077] 
\draw    (122.8,225) -- (257.8,225) ;
\draw [shift={(260.8,225)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(119.8,225)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp028275738414681006] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,142.18) .. controls (365,134) and (371.63,127.36) .. (379.82,127.36) .. controls (388,127.36) and (394.64,134) .. (394.64,142.18) .. controls (394.64,150.37) and (388,157) .. (379.82,157) .. controls (371.63,157) and (365,150.37) .. (365,142.18) -- cycle ;
%Curve Lines [id:da7202837492936005] 
\draw    (343.8,77.36) .. controls (279.45,122.9) and (302.33,173.34) .. (342.58,204.43) ;
\draw [shift={(343.8,205.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4678251099443136] 
\draw    (365,142.18) -- (288.45,89.5) ;
\draw [shift={(286.8,88.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Axis 2D [id:dp8494447421977243] 
\draw [line width=1.5]  (472,195.73) -- (648.8,195.73)(489.68,64) -- (489.68,210.36) (641.8,190.73) -- (648.8,195.73) -- (641.8,200.73) (484.68,71) -- (489.68,64) -- (494.68,71)  ;
%Shape: Right Triangle [id:dp441461564376495] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.25 ] (489,95) -- (610.8,196.36) -- (489,196.36) -- cycle ;
%Curve Lines [id:da691862389693042] 
\draw [line width=0.75]    (590.8,116.16) .. controls (573.16,147.52) and (568.97,116.46) .. (549.04,139.67) ;
\draw [shift={(547.8,141.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;
%Shape: Rectangle [id:dp29784833864235405] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (120.8,155.16) -- (260.8,155.16) -- (260.8,216.36) -- (120.8,216.36) -- cycle ;
%Straight Lines [id:da014819478856842094] 
\draw [line width=1.5]    (81.8,55.36) -- (260.8,55.36) ;
%Straight Lines [id:da19136676020039034] 
\draw [line width=1.5]    (80.8,115.36) -- (260.8,116.36) ;
%Straight Lines [id:da019274737615810222] 
\draw    (61.8,85.36) -- (89.8,85.36) ;
\draw [shift={(91.8,85.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43759945225025065] 
\draw [line width=1.5]    (260.8,55.36) -- (260.8,116.36) ;
%Shape: Rectangle [id:dp8414125012045715] 
\draw  [color={rgb, 255:red, 95; green, 19; blue, 254 }  ,draw opacity=0.23 ][fill={rgb, 255:red, 95; green, 19; blue, 254 }  ,fill opacity=0.23 ] (180.8,55.16) -- (260.8,55.16) -- (260.8,116.36) -- (180.8,116.36) -- cycle ;

% Text Node
\draw (8,176) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% Text Node
\draw (7,76) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% Text Node
\draw (206,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% Text Node
\draw (167,241) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% Text Node
\draw (361,100.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% Text Node
\draw (457,65.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% Text Node
\draw (623,196.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% Text Node
\draw (567,94.4) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\lambda _{1} +\lambda _{2} =1$};


\end{tikzpicture}

% \begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
% %uncomment if require: \path (0,240); %set diagram left start at 0, and has height of 240

% %Straight Lines [id:da09715700995858345] 
% \draw    (85.8,140.36) -- (264.8,139.36) ;
% %Straight Lines [id:da8887479227991981] 
% \draw    (85.8,198.36) -- (265.8,199.36) ;
% %Straight Lines [id:da8614120669050047] 
% \draw    (264.8,139.36) -- (265.8,199.36) ;
% %Straight Lines [id:da6217209993953612] 
% \draw    (54.8,169.36) -- (82.8,169.36) ;
% \draw [shift={(84.8,169.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4398173253440574] 
% \draw    (84.8,40.36) -- (263.8,39.36) ;
% %Straight Lines [id:da5015891688166809] 
% \draw    (84.8,98.36) -- (264.8,99.36) ;
% %Straight Lines [id:da875509031522369] 
% \draw    (263.8,39.36) -- (264.8,99.36) ;
% %Straight Lines [id:da6528587077790915] 
% \draw    (53.8,69.36) -- (81.8,69.36) ;
% \draw [shift={(83.8,69.36)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Rounded Rect [id:dp4517176185326244] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (156.8,53.67) .. controls (156.8,47.78) and (161.58,43) .. (167.47,43) -- (250.33,43) .. controls (256.22,43) and (261,47.78) .. (261,53.67) -- (261,85.69) .. controls (261,91.58) and (256.22,96.36) .. (250.33,96.36) -- (167.47,96.36) .. controls (161.58,96.36) and (156.8,91.58) .. (156.8,85.69) -- cycle ;
% %Rounded Rect [id:dp225981923335425] 
% \draw  [color={rgb, 255:red, 81; green, 74; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (105.8,153.67) .. controls (105.8,147.78) and (110.58,143) .. (116.47,143) -- (252.33,143) .. controls (258.22,143) and (263,147.78) .. (263,153.67) -- (263,185.69) .. controls (263,191.58) and (258.22,196.36) .. (252.33,196.36) -- (116.47,196.36) .. controls (110.58,196.36) and (105.8,191.58) .. (105.8,185.69) -- cycle ;
% %Straight Lines [id:da37671038244024846] 
% \draw    (156,29) -- (260.8,29) ;
% \draw [shift={(263.8,29)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(153,29)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Straight Lines [id:da0678614898035077] 
% \draw    (111.8,209) -- (263.8,209) ;
% \draw [shift={(266.8,209)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% \draw [shift={(108.8,209)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
% %Shape: Circle [id:dp028275738414681006] 
% \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.67 ] (365,126.18) .. controls (365,118) and (371.63,111.36) .. (379.82,111.36) .. controls (388,111.36) and (394.64,118) .. (394.64,126.18) .. controls (394.64,134.37) and (388,141) .. (379.82,141) .. controls (371.63,141) and (365,134.37) .. (365,126.18) -- cycle ;
% %Curve Lines [id:da7202837492936005] 
% \draw    (343.8,61.36) .. controls (279.45,106.9) and (302.33,157.34) .. (342.58,188.43) ;
% \draw [shift={(343.8,189.36)}, rotate = 217.09] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Straight Lines [id:da4678251099443136] 
% \draw    (365,126.18) -- (288.45,73.5) ;
% \draw [shift={(286.8,72.36)}, rotate = 394.53999999999996] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Axis 2D [id:dp8494447421977243] 
% \draw [line width=1.5]  (461,179.73) -- (637.8,179.73)(478.68,48) -- (478.68,194.36) (630.8,174.73) -- (637.8,179.73) -- (630.8,184.73) (473.68,55) -- (478.68,48) -- (483.68,55)  ;
% %Shape: Right Triangle [id:dp441461564376495] 
% \draw  [fill={rgb, 255:red, 74; green, 120; blue, 226 }  ,fill opacity=0.6 ] (478,79) -- (599.8,180.36) -- (478,180.36) -- cycle ;
% %Curve Lines [id:da691862389693042] 
% \draw [line width=0.75]    (579.8,100.16) .. controls (562.16,131.52) and (557.97,100.46) .. (538.04,123.67) ;
% \draw [shift={(536.8,125.16)}, rotate = 308.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-4.9) .. controls (6.95,-2.3) and (3.31,-0.67) .. (0,0) .. controls (3.31,0.67) and (6.95,2.3) .. (10.93,4.9)   ;

% % Text Node
% \draw (8,160) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{2}( t)$};
% % Text Node
% \draw (7,60) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{1}( t)$};
% % Text Node
% \draw (186,5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{1}( t)$};
% % Text Node
% \draw (169,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Q_{2}( t)$};
% % Text Node
% \draw (361,88.4) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{D}( t)$};
% % Text Node
% \draw (446,49.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{2}$};
% % Text Node
% \draw (612,180.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1}$};
% % Text Node
% \draw    (526,68) -- (635,68) -- (635,99) -- (526,99) -- cycle  ;
% \draw (529,72.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\lambda _{1} +\lambda _{2} \leq 1$};
% % Text Node
% \draw (461,175.4) node [anchor=north west][inner sep=0.75pt]  [font=\Large]  {$o$};


%\end{tikzpicture}
}
